Propositional Abduction with Implicit Hitting Sets

Logic-based abduction finds important applications in artificial intelligence and related areas. One application example is in finding explanations for observed phenomena. Propositional abduction is a restriction of abduction to the propositional domain, and complexity-wise is in the second level of the polynomial hierarchy. Recent work has shown that exploiting implicit hitting sets and propositional satisfiability (SAT) solvers provides an efficient approach for propositional abduction. This paper investigates this earlier work and proposes a number of algorithmic improvements. These improvements are shown to yield exponential reductions in the number of SAT solver calls. More importantly, the experimental results show significant performance improvements compared to the the best approaches for propositional abduction.

==> apdx.tex <==
%------------------------------------------------------------------------------%
% File:        apdx.tex
%
% Description: 
%
% Created:     13 Apr 2016.
%
% Author:      Joao Marques-Silva (jpms).
%------------------------------------------------------------------------------%

\subsection*{Appendix}

Example of an abduction instance:

The example considers 
$T=\{(\neg x_1 \vee x_4), (\neg x_2 \vee \neg x_3 \vee x_4)\}$, 
$H = \{(x_1), (x_2), (x_3)\}$, and
$M = \{x_4\}$.

The solution for this example is $S = \{(x_1)\}$.

Given the set of assumptions $A = \{a_1, a_2, a_3\}$ associated to the hypothesis, the QBF formula for testing is:
$$ 
\begin{array}{l}
	\exists_{x_1, x_2, x_3, x_4}
	\\ 
	(\neg x_1 \vee x_4) (\neg x_2 \vee \neg x_3 \vee x_4)
	(x_1 \vee a_1) (x_2 \vee a_2) (x_3 \vee a_3) 
	\\
	\forall_{y_1, y_2, y_3, y_4}
	\\
	\neg [
	(\neg y_1 \vee y_4) (\neg y_2 \vee \neg y_3 \vee y_4)
	(y_1 \vee a_1) (y_2 \vee a_2) (y_3 \vee a_3)
	(\neg y4)]
\end{array}
$$ 

%------------------------------------------------------------------------------%


==> hyper.tex <==
%------------------------------------------------------------------------------%
% File:        beacon.tex
%
% Description:
%
% Created:     26 Feb 2016.
%
% Author:      Alexey Ignatiev (aign).
%------------------------------------------------------------------------------%

% block styles
\tikzstyle{small} = [rectangle,font=\scriptsize,rounded corners=1mm,thick,%
                     draw=black!80, top color=white,bottom color=blue!20,%
                     minimum height=.5cm,minimum width=.5cm,inner sep=2pt,draw%
                    ]
% Define block styles
\tikzstyle{block} = [rectangle,font=\scriptsize,rounded corners=1mm,thick,%
                     draw=black!80, top color=white,bottom color=blue!20,%
                     draw,text width=5.5em, minimum height=3.0em, text centered,%
                     inner sep=2pt%
                    ]
\tikzstyle{simple1} = [font=\scriptsize, text centered, text width=3em]
\tikzstyle{simple2} = [font=\small,      text centered]

% defining box structure
\tikzstyle{box} = [draw=black!90, thick, rectangle, rounded corners,
    inner sep=10pt, inner ysep=20pt, dashed,top color=white,bottom color=green!5]
\tikzstyle{title} = [draw=black!90, fill=black!5, thick, top color=white,
                     bottom color = black!5, text=black!90, rectangle,font=\small
                    ]

\begin{tikzpicture}[node distance = 5.0em, auto]
    % creating a box with the title
    \node [box] (box) {%
      \begin{minipage}[t!]{0.4\textwidth}
        \vspace{1.0cm}\hspace{4cm}
      \end{minipage}
    };
    \node[title] at (box.south) {Hyper};

    % nodes
    \node [simple2, yshift=1.6cm      ] (input)      {$P=(V,H,M,T,c)$};
    \node [simple2, below of=input, yshift=0.6cm    ] (relax)      {$(H',R)\gets\relaxcls(H)$};
    \node [simple2, below of=relax, yshift=1.2cm    ] (ba)          {$B\gets T\land M\land H'$ and $A\gets \emptyset$};
    \node [block, below left  of=ba, yshift=-0.3cm,xshift=-0.6cm] (maxsat)     {MaxSAT solver $MHS(A,B)$};
    \node [block, below right of=ba, yshift=-0.3cm,xshift=0.6cm] (sat)        {SAT solver $T\land S\land(\neg{M})$};
    \node [simple2, yshift=-2.6cm      ] (output)      {output};
    % \node [block                 ] (horn) at (-3,0)   {Classification + Horn encoding};
    % \node [simple2, left  of=horn] (t)      {$tbox$};
    % \node [simple2, above of=horn, yshift=-0.1cm] (tprime) {$tbox'$};
    % \node [simple2, right of=horn] (h)      {$\fml{H}$};
    % \node [block,   right of=h   ] (ghorn)  {Group Horn formula generation and reduction};
    % \node [simple2, above of=ghorn, yshift=-0.1cm] (subs) {$C \sqsubseteq_{\fml{T}} D$};
    % \node [simple2, right of=ghorn] (hg)     {$\fml{H}_G$};
    % \node [small,   above right of=hg, yshift=-0.5cm] (hgmus)  {\textsc{HgMUS}};
    % \node [simple1, right of=hgmus] (minas)  {MinAs diagnoses};
    % \node [small,   below right of=hg, yshift=0.5cm] (forqes) {\textsc{Forqes}};
    % \node [simple1, right of=forqes] (smus)   {Smallest MinAs};

    % edges
    \draw [->,thick,black!80] (input)      -- (relax);
    \draw [->,thick,black!80] (ba)         -- (maxsat);
    \draw [->,thick,black!80] (ba)         -- (sat);
    \draw [->,thick,black!80,transform canvas={yshift=-0.3cm}] (maxsat)     -- (sat);
    \draw [->,thick,black!80] (maxsat) node[near start,below] {$\emptyset$}    -- (output);
    \draw [->,thick,black!80,transform canvas={yshift=0.3cm}] (sat)        -- (maxsat);
    \draw [->,thick,black!80] (sat) node[near start,below] {$S$}    -- (output);
    % \draw [->,thick,black!80] (t)      -- (horn);
    % \draw [->,thick,black!80] (horn)   -- (tprime);
    % \draw [->,thick,black!80] (horn)   -- (h);
    % \draw [->,thick,black!80] (h)      -- (ghorn);
    % \draw [->,thick,black!80] (subs)   -- (ghorn);
    % \draw [->,thick,black!80] (ghorn)  -- (hg);
    % \draw [->,thick,black!80] (hg)     -- (hgmus);
    % \draw [->,thick,black!80] (hgmus)  -- (minas);
    % \draw [->,thick,black!80] (hg)     -- (forqes);
    % \draw [->,thick,black!80] (forqes) -- (smus);
\end{tikzpicture}

%------------------------------------------------------------------------------%

